Can LLMs Generate Diverse Molecules? Towards Alignment with Structural Diversity

Recent advancements in large language models (LLMs) have demonstrated impressive performance in molecular generation, which offers potential to accelerate drug discovery. However, the current LLMs overlook a critical requirement for drug discovery: proposing a diverse set of molecules. This diversity is essential for improving the chances of finding a viable drug, as it provides alternative molecules that may succeed where others fail in real-world validations. Nevertheless, the LLMs often output structurally similar molecules. While decoding schemes like diverse beam search may enhance textual diversity, this often does not align with molecular structural diversity. In response, we propose a new method for fine-tuning molecular generative LLMs to autoregressively generate a set of structurally diverse molecules, where each molecule is generated by conditioning on the previously generated molecules. Our approach consists of two stages: (1) supervised fine-tuning to adapt LLMs to autoregressively generate molecules in a sequence and (2) reinforcement learning to maximize structural diversity within the generated molecules. Our experiments show that the proposed approach enables LLMs to generate diverse molecules better than existing approaches for diverse sequence generation.

==> 2_preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}


==> resources/compare_3300_sota.tex <==
\definecolor{whitegray}{RGB}{243, 243, 243} % This is a very light gray

\begin{table}[t]
\caption{\textbf{Comparison with existing LLMs on description-based molecule generation.} Our method shows superior performance compared to the considered baselines. }\label{tab:sota}
\centering
{
\scalebox{0.97}{\begin{tabular}{lccccc}
\toprule
Method & Accepted \& Unique & NCircles$_{h=0.25}$ & NCircles$_{h=0.35}$ & IntDiv. & Top 10 \\
\midrule
\rowcolor{whitegray} \multicolumn{6}{l}{\textit{Single-task Specialist LLMs}} \\
%T5 & \\ 
MolT5 \citep{xx} & 3.44 & 1.93 & 1.58 & 0.14 & 0.44 \\
Text+Chem T5 \citep {xx} & 3.73 & 0.99 & 0.76 & 0.06 & 0.20 \\
BioT5 \citep{xx} & 15.94 & 8.27 & 6.15 & 0.30 & 0.68\\
BioT5$^{+}$ \citep{xx} & 16.22 & 8.02 & 6.20 & 0.32 & 0.65 \\
\midrule
\textbf{BioT5$^{+}$+ours} & \textbf{21.61} & \textbf{16.53} & \textbf{13.85} & \textbf{0.44} & \textbf{0.73} \\
\bottomrule
\end{tabular}}
}
\end{table}

==> resources/compare_search_MolT5.tex <==
\begin{figure}[t]
\centering
  \includegraphics[width=0.96\linewidth]{resources/figures/MolT5_subplot.pdf}\;
\caption{\textbf{Comparison with decoding schemes on MolT5.} Our method generates more diverse and promising molecules compared to the baselines. Notably, our method makes a larger gap over the baselines on metrics related to capturing both quality and diversity, i.e., NCircles.}\label{fig:molt5_main}
\end{figure}

==> resources/fig_llm_molecule.tex <==
\begin{figure}
%\vspace{-.05in}
\centering
\includegraphics[width=0.85\linewidth]{resources/figures/molgen.pdf}\;
\caption{\textbf{LLMs generate a molecule with SMILES representation.}}\label{fig:molgen}
\vspace{-.15in}
\end{figure}

%\begin{wrapfigure}{r}{0.35\textwidth}
%\vspace{-.1in}
%\centering
%    \includegraphics[width=0.98\linewidth]{resources/figures/drug_discovery.pdf}
%\caption{\textbf{ddd.} }\label{fig:drugdiscovery}
%\vspace{-.1in}
%\end{wrapfigure}

==> resources/fig_pipelien.tex <==
%\begin{wrapfigure}{r}{0.35\textwidth}
%\vspace{-.1in}
%\centering
%    \includegraphics[width=0.98\linewidth]{resources/figures/drug_discovery.pdf}
%\caption{\textbf{ddd.} }\label{fig:drugdiscovery}
%\vspace{-.1in}
%\end{wrapfigure}

\begin{figure*}[h]
\centering  \includegraphics[width=0.94\textwidth]{resources/figures/pipelin2.pdf}
  \vspace{-.07in}
\caption{\textbf{The compute-aided drug design.} A collection of structurally diverse molecules is required to increase the chance of identifying viable drug candidates in the real world.}\label{fig:drugdiscovery}
\vspace{-.05in}
\end{figure*}

==> resources/tab_vis.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.245\linewidth}
\centering
  \includegraphics[width=\linewidth]{resources/figures/plot_0.pdf}
  \subcaption{BS \\ \small{(22,11)}}
\end{subfigure}
\begin{subfigure}[t]{0.245\linewidth}
\centering
  \includegraphics[width=\linewidth]{resources/figures/plot_1.pdf}
  \subcaption{Diverse BS \\ \small{(7,4)}}
\end{subfigure}
\begin{subfigure}[t]{0.245\linewidth}
\centering
  \includegraphics[width=\linewidth]{resources/figures/plot_2.pdf}
  \subcaption{Contrastive BS\\ \small{(26, 11)}}
\end{subfigure}
\begin{subfigure}[t]{0.245\linewidth}
\centering
  \includegraphics[width=\linewidth]{resources/figures/plot_3.pdf}
  \subcaption{Div-SFT+RL\\ \small{(29,28)}}
\end{subfigure}
\caption{\textbf{The distribution of (Accepted \& unique, NCircles$_{h=0.65}$) obtained by each method.} The molecules are generated from the description in \Cref{tab:ex_biot5}. The Fruchterman-Reingold force-directed algorithm \citep{fruchterman1991graph} embeds each molecule in a 2-dimensional space based on Tanimoto similarity. Here, a low distance yields a high Tanimoto similarity. Each dot, shaded circle, and edge represent accepted molecules, \textcolor{blue}{a boundary for determining similar or distinct molecules}, and a pair with similarity above $0.65$, respectively. Our method better captures the molecular diversity.}\label{fig:vis}
\vspace{-.2in}
\end{figure*}
